Optimal Offline and Competitive Online Strategies for Transmitter-Receiver Energy Harvesting

Transmitter-receiver energy harvesting model is assumed, where both the transmitter and receiver are powered by random energy source. Given a fixed number of bits, the problem is to find the optimal transmission power profile at the transmitter and ON-OFF profile at the receiver to minimize the transmission time. Structure of the optimal offline strategy is derived together with an optimal offline policy. An online policy with competitive ratio of strictly less than two is also derived.

==> Algo1_proofICC.tex <==
%!TEX root = OptimalOfflineICC.tex
%input{Siddhartha}


%\begin{algorithm}
%\caption{Off-line Algorithm for finding optimal transmission policy to Problem 1}
%\footnotesize%\scriptsize
%\label{Algorithm1}
%\begin{algorithmic}[1]
%\State \textbf{Initialization}: $\{\textbf{p},\textbf{s},N\}\gets$ INIT\_POLICY
%\State $t_l=s_2$, $t_{r}=s_{N}$, $T_{start}=s_1$, $T_{stop}=s_{N+1}$, $p_l=p_1$, $p_r=p_{N}$, $control=0$.
%\State Delete $s_1$, Delete $s_{N+1}$, Delete $p_N$, Delete $p_1$.
%%\Procedure{InitPolicy}{}
%\While {$\left(T_{stop}-T_{start}< \TRx_0\right) \text{ and } \left(T_{start}>0\right)$}
%\label{algo_while_loop}
%	\If {$\{i:t_r<t_i < T_{stop}\}=\emptyset$}
%		\State $B_l=g(p_r)(T_{stop}-t_r)+g(p_l)(t_l-T_{start})$, $control=1$.
%	\Else
%		\State $j=\displaystyle \argmin_{i:t_r<t_i < T_{stop}} \mathcal{P}(t_r,t_i)$
%		\State $B_l=g(p_r)(T_{stop}-t_r)+g(p_l)(t_l-T_{start})-g\left(\mathcal{P}(t_r,t_j)\right)						\left(\frac{\ETx(T_{stop}^-)-\ETx(t_r^-)}{\mathcal{P}(t_r,t_j)}\right) $\label{algo_bits_left_1}
%	\EndIf
%
%	\State Solve for $\tilde{p}$: $\frac{\ETx(t_l^-)}{\tilde{p}}g(\tilde{p})=B_l$\label{algo_bits_left_2}
%	\State $A=\{i:\tilde{p}t_i+(\ETx(t_l^-)-\tilde{p}t_l))> \ETx(t_i^-), \forall \left(t_l-					\frac{\ETx(t_l^-)}{\tilde{p}}\right)<t_i<t_l\}$
%
%	\If {$A=\emptyset$}
%		\State $p_l=\tilde{p}$, $T_{start}=t_l-\ETx(t_l^-)/p_l$
%		\If {$control=0$}
%			\State $p_r=\mathcal{P}(t_r,t_j)$, $T_{stop}=t_r+\frac{\ETx(T_{stop^-})-\ETx(t_r^-)}							{\mathcal{P}					(t_r,t_j)}$
%			\State $t_r=t_j$, $\textbf{p}.append(\mathcal{P}(t_r,t_j))$, $\textbf{s}.append( t_j)$ 
%		\Else
%			\State $T_{stop}=t_r$, $t_r=\textbf{s}.last$, $p_r=\textbf{p}.last$
%			\State Delete $\textbf{s}.last$, Delete $\textbf{p}.last$
%			\State $control=0$
%		\EndIf
%	\Else 
%		\State $k=\displaystyle \argmax_{i:\max\left(\left(t_l-\ETx(t_l^-)/\tilde{p}\right),0\right)					\le t_i <t_l} \mathcal{P}(t_i,t_l)$
%		\State $B_r=g(p_r)(T_{stop}-t_r)+g(p_l)(t_l-T_{start})-g\left(\mathcal{P}(t_k,t_l)\right)							\left(\frac{\ETx(T_{start}^-)}{\mathcal{P}(t_k,t_l)}\right)$
%		\State $p_l=\mathcal{P}(t_k,t_l)$, $T_{start}=t_l-\ETx(t_l^-)/\mathcal{P}(t_k,t_l)$
%		 
%		\State $t_l=t_k$, $\textbf{p}.prepend=p_l$, $\textbf{s}.prepend=t_k$
%	
%		\State Solve for $p_r$: $\frac{\ETx(T_{stop}^-)-\ETx(t_r)}{p_r}g(p_r)=B_r$
%		\State $T_{stop}=t_r+(\ETx(T_{stop}^-)-\ETx(t_r^-))/p_r$	
%	\EndIf
%
%\EndWhile
%
%\If {$(T_{start}-T_{stop})>\TRx_0$}
%	\State $T=\TRx_0-(t_r-t_l)$, $B=B_0-\displaystyle\sum_{i}g(p_i)(s_{i+1}-s_{i})$
%	\State Solve for  $x$: $xg\left(\dfrac{\ETx(t_{l}^-)}{x}\right)+\left(T-x\right) g 		\left(\dfrac{\ETx(t_{stop}^-)-\ETx(t_{r}^-)}{T-x}\right) = B$(with prev iteration $t_l$ and $t_r$)\label{algo_solve_eqn}
%	\State $p_l=\dfrac{\ETx(t_{l}^-)}{x}$, $T_{start}=t_l-x$
%	\State $p_r=\dfrac{\ETx(t_{stop}^-)-\ETx(t_{r}^-)}{T-x}$, $T_{stop}=t_r+T-x$
%\EndIf
%
%\State $\textbf{p}.prepend(p_l)$, $\textbf{s}.prepend(T_{start})$, $\textbf{p}.append(p_r)$, $\textbf{s}.append(T_{stop})$
%\State \Return $\{\textbf{p},\textbf{s}, \text{number of elements in \textbf{p}}\}$ 	 
%%\EndProcedure
%\end{algorithmic}
%\end{algorithm}


%\begin{proof}

%The proof consists of establishing both necessary and sufficiency conditions. First we work out the necessary part i.e. an optimal policy, say $X$, $\{\textbf{p},\textbf{s},N\}$ must have the given structure. We prove it by contradiction. We establish structure (\ref{claim3}) at first. Assume the optimal policy $X$ satisfies Lemmas \ref{lemma_increasing_power}-\ref{lemma_Q} and does not satisfy structure (\ref{claim3}). Specifically, say the policy abides by the  structure (\ref{claim3}) from time $s_{1}$ to $s_n$, for some $n\in \{1,2,..,N\}$ but transmission power right after $s_n$ is not the minimum feasible constant power, i.e.
%\begin{align}
%p_n>\mathcal{P}(s_n,\tilde{s})\text{ where } \tilde{s}=\argmin_{t_i: s_n < t_i \le s_{N+1}} \mathcal{P}(t_i,s_n).\label{claim3_1}
%\end{align}
%Note that $p_n$ is not less than $\mathcal{P}(s_n,\tilde{s})$, as $\mathcal{P}(s_n,\tilde{s})$ is the minimum feasible power among all the epochs. The maximum energy that can used for transmission from time $s_{n}$ to $\tilde{s}$ is $\left(\ETx(\tilde{s}^-)-\ETx(s_{n}^-)\right)$, since the optimal policy has used all the energy till time $s_{n}^-$, by Lemma \ref{lemma_energy_consumed}. If $\tilde{s}<s_{n+1}$, the transmission policy uses $p_n(\tilde{s}-s_{n})$ energy from time $s_n$ to $\tilde{s}$. If $\tilde{s}>s_{n+1}$, the transmission power during time $[s_{n+1},\tilde{s}]$ has to be greater than or equal to $p_n$ by Lemma \ref{lemma_increasing_power}. So the total energy used during period $[s_n,\tilde{s}]$ can be lower bounded by $p_n(\tilde{s}-s_{n})$. But, this energy is always more than the maximum energy available from $s_{n}$ to $\tilde{s}$ because
%\begin{align}
%&\nonumber\ETx(\tilde{s}^-)-\ETx(s_{n}^-)=\mathcal{P}(s_n,\tilde{s})(\tilde{s}-s_{n})<p_n(\tilde{s}-s_{n}),
%\end{align}
%where the inequality follows from (\ref{claim3_1}). This violates constraint (\ref{pb1_constraint_energy}) and contradicts the optimality of $X$.
%
%Moving on to other structures, (\ref{claim1}) must be followed by the optimal policy as it is a constraint to the Problem 1, (\ref{claim4}) follows from Lemma \ref{lemma_Q} and \eqref{claim2} follows from Lemma \ref{transmission_duration}.


%The proof consists of establishing both necessary and sufficiency conditions. First we work out the necessary part i.e. an optimal policy must have the given structure. Observing the structure, (\ref{claim1}) must be followed by the optimal policy as it is a constraint to the Problem 1, \eqref{claim3} follows from Lemma \ref{lemma_increasing_power}, \ref{lemma_nobreaks}, \eqref{claim4} follows from Lemma \ref{lemma_energy_consumed}, \eqref{claim2} follows from Lemma \ref{transmission_duration} and \eqref{claim5} follows from Lemma \ref{lemma_Q}.
%
%
%
%%We are left to prove structure (\ref{claim2}). $s_{N+1}-s_1\le \mathcal{R}_0$ by constraint (\ref{pb1_constraint_time}). If $s_1=0$ then we are done. When $s_1>0$, assume that $s_{N+1}-s_1<\mathcal{R}_0$. Now consider the policy where power vector is given by $\bm{\widetilde{p}}=\{p_1-\alpha,p_2,..,p_{N-1},p_N+\beta \}$ and the corresponding time vector be given by $\bm{\widetilde{s}}=\{s_1-\gamma,s_2,..,s_{N},s_{N+1}-\delta\}$, where $\gamma=\dfrac{\alpha}{p_1-\alpha}(s_2-s_1)$, $\delta =\dfrac{\beta}{p_N+\beta}(s_{N+1}-s_N)$ and $\alpha ,\beta$ are small positive constants. Since $(s_{N+1}-\delta)>s_{N+1}$, this policy finishes before the optimal policy $\{\textbf{p},\textbf{s},N\}$ and hence amounts to a contradiction only if we are able to show that it is feasible. By the definition of $s_i$ in (\ref{claim3}), $s_{2}$ is the first energy arrival which is on the boundary of energy constraint (\ref{pb1_constraint_energy}) i.e. $U(s_2)=\ETx(s_2^-)$ and $s_{N}$ is the last epoch satisfying $U(s_N)=\ETx(s_N^-)$. So we can choose arbitrarily small $\alpha ,\beta$ such that policy $\{\bm{\widetilde{p}},\bm{\widetilde{s}},N\}$ would be feasible with respect energy constraint (\ref{pb1_constraint_energy}). For every $\beta\rightarrow 0^+$ we can find a value of $\alpha$ such that the number of bits transmitted in policy $\{\bm{\widetilde{p}},\bm{\widetilde{s}},N\}$ remains the same as policy $\{\textbf{p},\textbf{s},N\}$ i.e. equal to $B_0$. So, excluding the common parts in the transmission policy $\{\textbf{p},\textbf{s},N\}$ and $\{\bm{\widetilde{p}},\bm{\widetilde{s}},N\}$, we can equate
%%\begin{align}
%%&g(p_N)(s_{N+1}-s_N)+g(p_1)(s_2-s_1)\nonumber
%%\\
%%&=g(p_1-\alpha)(s_2-s_1+\gamma)+g(p_N+\beta)(s_{N+1}-s_N-\delta)\nonumber,
%%\\
%%&\implies \delta(p_N+\beta)p_N\frac{1}{\beta}\left(\frac{g(p_N)}{p_N}-\frac{g(p_N+\beta)}{p_N+\beta}\right)\nonumber
%%\\
%%&=\gamma(p_1-\alpha)p_1\frac{1}{\alpha}\left(\frac{g(p_1-\alpha)}{p_1-\alpha}-\frac{g(p_1)}{p_1}\right).\label{bits_equal}
%%\end{align}
%%$\exists$ $p_N':p_N<p_N'<p_{N}+\beta$ and $p_1':p_1-\alpha<p_1'<p_{1}$ such that
%%\begin{align}
%%&\frac{d}{dp} \frac{g(p)}{p} \bigg{\vert}_{p=p_N'}=\frac{1}{\beta}\left(\frac{g(p_N+\beta)}{p_N+\beta}-\frac{g(p_N)}{p_N}\right),\label{diff_1}
%%\\
%%&\frac{d}{dp} \frac{g(p)}{p}\bigg{\vert}_{p=p_1'}=-\frac{1}{\alpha}\left(\frac{g(p_1-\alpha)}{p_1-\alpha}-\frac{g(p_1)}{p_1}\right)\label{diff_2}.
%%\end{align}
%%Substituting (\ref{diff_1}) and (\ref{diff_2}) into (\ref{bits_equal}) we get,
%%\begin{align}
%%&\delta(p_N+\beta)p_N\frac{d}{dp} \frac{g(p)}{p}  \bigg{\vert}_{p=p_N'}
%%=\gamma(p_1-\alpha)p_1\frac{d}{dp} \frac{g(p)}{p} \bigg{\vert}_{p=p_1'}.\label{bits_equal1}
%%\end{align}
%%It can be verified that $\dfrac{d}{dp} \dfrac{g(p)}{p}$ is decreasing function of $p$. As $p_1'<p_N'$, equation (\ref{bits_equal1}) implies $\gamma >\delta$. Hence the time for which transmission occurs in the policy $\{\bm{\widetilde{p}},\bm{\widetilde{s}},N\}$, $\left( s_{N+1}-s_1+\gamma-\delta\right)$, is greater than transmission time in policy $\{\textbf{p},\textbf{s},N\}$ i.e. $(s_{N+1}-s_1)$. As $s_{N+1}-s_1<\TRx_0$, we can choose arbitrarily small positive value of $\beta$ so that $(s_{N+1}-s_1)<(s_{N+1}-s_1+\gamma -\delta)<\TRx_0$ holds. So policy $\{\bm{\widetilde{p}},\bm{\widetilde{s}},N\}$ is feasible with constraints  (\ref{pb1_constraint_bits}), (\ref{pb1_constraint_energy}), (\ref{pb1_constraint_time}) and contradicts the optimality of policy $\{\textbf{p},\textbf{s},N\}$. This concludes that $s_{N+1}-s_1=\TRx_0$ (if $s_1\neq 0$) in optimal policy.
%
%Next, we prove the sufficiency of the structure. Let a policy $X$, $\{\textbf{p},\textbf{s},N\}$ follow  structure \eqref{claim1}-\eqref{claim5}. We need to show that this policy is optimal. We adopt the method of contradiction to prove this. Assume that it is not true. So, there exists another policy $Y$, $\{\textbf{p'},\textbf{s'},N'\}$ which is optimal. $Y$ abides by the Lemma \ref{lemma_increasing_power}-\ref{lemma_Q}, as $Y$ is optimal. Thus, $Y$ also follows structure \eqref{claim1}-\eqref{claim5}. Hence, our problem reduces to show that there cannot exist two different policies $X$ and $Y$ (of which $Y$ is optimal) satisfying structure \eqref{claim1}-\eqref{claim5}\footnote{Note that Lemma \ref{lemma_nobreaks} suggests that optimal solution to Problem 1 may not be unique in general, but Theorem \ref{th_algo1_1} shows that the optimal solution \textit{without breaks} in transmission is indeed unique.}.
%
%%\textit{Case1}: If $s_1'>s_1\ge 0$, then by Lemma \ref{transmission_duration}, $s_{N'+1}'=s_1'+\TRx_0>s_1+\TRx_0\ge s_{N+1}$. So policy $Y$ finishes after time $s_{N+1}$ and hence cannot be optimal. 
%
%\textit{Case1}: If $s_1'>s_1\ge 0$, then by \eqref{claim2}, $s_{N'+1}'=s_1'+\TRx_0>s_1+\TRx_0\ge s_{N+1}$. So policy $Y$ finishes after time $s_{N+1}$ and hence cannot be optimal. 
%
%\textit{Case2}: Suppose $s_1'=s_1$. Let $s_i'$ be the first epoch for which $p_i'\ne p_i$ for some $i \in \{1,2,..,N\}$. 
%%By \eqref{claim3}, since $p_i$ is the minimum possible power among all epochs, $p_i'>p_i$. 
%
%%Suppose $p_i'>p_i$. If, in policy $Y$, transmission continues after $s_{i+1}$ i.e. $s_{N'+1}'>s_{i+1}$, then the amount of energy used by $Y$ in interval $[s_{i},s_{i+1}]$ can be lower bounded by $p_i'(s_{i+1}-s_i)$ from Lemma \ref{lemma_increasing_power}. $p_i'(s_{i+1}-s_i)$ is more than $p_i(s_{i+1}-s_i)$, which is the energy used by policy $X$. But by structure \eqref{claim4}, $X$ uses all energy available by $s_{i+1}$. So $Y$ uses more than available energy in $[s_{i},s_{i+1}]$ and is not feasible with respect to the energy constraint. 
%
%Suppose $p_i'>p_i$. If, in policy $Y$, transmission continues after $s_{i+1}$ i.e. $s_{N'+1}'>s_{i+1}$, then the amount of energy used by $Y$ in interval $[s_{i},s_{i+1}]$ can be lower bounded by $p_i'(s_{i+1}-s_i)$ from \eqref{claim3}. $p_i'(s_{i+1}-s_i)$ is more than $p_i(s_{i+1}-s_i)$, which is the energy used by policy $X$. But by structure \eqref{claim4}, $X$ uses all energy available by $s_{i+1}$. So $Y$ uses more than available energy in $[s_{i},s_{i+1}]$ and is not feasible with respect to the energy constraint. 
%
%If $s_{N'+1}'\le s_{i+1}$, then it can be easily verified by (\ref{property_decreasing}) that $Y$ transmits strictly less number of bits in interval $[s_i,s_{N'+1}]$ than $X$ in interval $[s_{i},s_{i+1}]$. Both policies being same till $s_i$, we conclude that $Y$ transmits less than $B_0$ bits and thus it is not feasible.
%
%When $p_i>p_i'$, symmetrical arguments follow.
%
%\textit{Case3}: This case argues the infeasibility when $s_1'<s_1$. Unlike other cases this case is more laborious. The idea of the proof is to show that if a optimal policy starts its transmission early and finishes earlier than policy $X$, it always takes more transmission time, which is going to violate the time constraint (\ref{pb1_constraint_time}). First, we establish that the $Y$ must be same as policy $X$ from epoch $s_2$ to an epoch $s_j$ such that $s_j=\displaystyle\max_{s_i<s_{N'+1}'} s_i$. Let $s_k'=\displaystyle\max_{s_i'<s_2}s_i'$, and transmission continue with constant power $p_k'$ till $s_{k+1}'$. Clearly $s_{k+1}'\ge s_2$. 
%
%If $s_{k+1}'>s_2$, transmission with a constant power $\dfrac{\ETx(s_{k+1}'^-)}{(s_{k+1}'-s_1)} $ from $s_1$ to $s_{k+1}'$ is feasible (as $p_k'$ is feasible) and $\dfrac{\ETx(s_{k+1}'^-)}{(s_{k+1}'-s_1)}<\dfrac{\ETx(s_2^-)}{(s_2-s_1)}=p_1$. 
%%This contradicts ($\ref{claim3}$), as $p_1$, no longer remains the minimum power. So, $s_{k+1}'=s_2$. Now, let $p_{k+1}'\neq p_2$ and $s_j>s_3$. From definition of $p_2$, $p_{k+1}>p_2$. Then the amount of energy used by policy $Y$ between $s_2$ and $s_3$ is more than what is harvested. So $p_{k+1}'=p_2$ ($s'_{k+2}=s_3$) and similarly, we can show that $p'_{k+2}=p_3$.. ($ s'_{k+3}=s_4$..) till epoch $s_j$. By structure (\ref{claim5}) and Lemma \ref{lemma_Q} we can be sure that there exists atleast one epoch $s_i=t_q$ which belongs to $\textbf{s}$ as well as $\textbf{s'}$, respectively, i.e. $j\ge 2$.
%Since $s_{N+1}=s_1+\TRx_0>s_1'+\TRx_0\ge s'_{N'+1}\ge s'_{k+1}$, $X$ exists in interval $[s_1,s'_{k+1}]$. $X$ uses atleast $p_1(s'_{k+1}-s_2)$ energy in this interval by \eqref{claim3}. But $\dfrac{\ETx(s_{k+1}'^-)}{(s_{k+1}'-s_1)}<p_1$. Hence $X$ uses more than available energy in $[s_1,s'_{k+1}]$. So, $s_{k+1}'=s_2$. Now, let $p_{k+1}'\neq p_2$ and $s_j>s_3$. From definition of $p_2$, $p_{k+1}>p_2$. Then the amount of energy used by policy $Y$ between $s_2$ and $s_3$ is more than what is harvested. So $p_{k+1}'=p_2$ ($s'_{k+2}=s_3$) and similarly, we can show that $p'_{k+2}=p_3$.. ($ s'_{k+3}=s_4$..) till epoch $s_j$. By structure (\ref{claim5}) we can be sure that there exists atleast one epoch $s_i=t_q$ which belongs to $\textbf{s}$ as well as $\textbf{s'}$, respectively, i.e. $j\ge 2$.
%
%\begin{figure}[htb]
%\centering
%\centerline{\includegraphics[width=8cm]{Theorem1_sufficient.pdf}}
%\caption{Energy curves at Transmitter explaining \textit{Case3} in proof of Theorem \ref{th_algo1_1}}
%\label{Theorem1_figure}
%\end{figure}
%
%Now, consider the following process which creates feasible policies from policy $\{\textbf{p'},\textbf{s'},N'\}$ as shown in Fig. \ref{Theorem1_figure}. We define two pivots $l$ and $r$. Initially we set $l=s_2'$ and $r=s_{N'}'$. The transmission power right before $l$ is $u$ ($u=p_1'$ initially) and right after $r$ is $v$ ($v=p_{N'}'$ initially). Keeping the policy same from $l$ to $r$ we increase $u$ by a small amount to $u+du$ and decrease $v$ by a small amount to $v-dv$ such that the number of bits transmitted (i.e. $B_0$) remains same under this transformation. Let $s_1'$ change to $s_1'+x$ and $s_{N'+1}'$ change to $s_{N'+1}'+y$ for some $x,y>0$ (Note that $y$ is dependent on $x$). We denote such a policy by vectors $\{\textbf{p'(x)},\textbf{s'(x)},N'(x)\}$. Following Lemma \ref{lemma_increase_time}, we can conclude that $(s_{N'(x)+1}'(x)-s_1'(x))<(s_{N'+1}'-s_1')$. We continue increasing $x$ till either $u=p_2$ (in which case we change $l=s_2$) or $v=p_{N'-1}'$ (where we change $r=s_{N'-1}'$) or $s_{N'(x)+1}'(x)$ hits an epoch, say $t_j$ ($r=t_j$, $v\rightarrow\infty$ in this case). After this, we again start increasing $x$ with changed definitions. We continue this process till $x=s_1-s_1'$  or $u$ becomes equal to $v$. Note that the former stopping criteria will be met at a smaller $x$ than the later one since policy $\{\textbf{p'(x)},\textbf{s'(x)},N'(x)\}$ shares at least one epoch with policy $X$, by arguments of previous paragraph. By maintaining these rules we ensure that policy $\{\textbf{p'(x)},\textbf{s'(x)},N'(x)\}$ abides by structure \eqref{claim1}, \eqref{claim3}-\eqref{claim5} and is feasible with energy constraint. Since $\left( s_{N'(x)+1}'(x)-s_1'(x)\right)$ is decreasing with $x$, the policy is also feasible with time constraint. As this is continuous on $x$, at $x=s_1-s_1'$ we reach a policy such that $s_1'(x)=s_1$. For $x=s_1-s_1'$, if $s_{N'(x)+1}'(x)\ge s_{N+1}$ then $s_{N'+1}'-s_1'>s_{N'(x)+1}'(x)-s_1'(x)\ge s_{N+1}-s_1=\TRx_0$ and policy $Y$ is infeasible with time constraint. If $s_{N'(x)+1}'(x)< s_{N+1}$ then we can follow the arguments in \textit{Case2} to show that policy $\{\textbf{p'(x)},\textbf{s'(x)},N'(x)\}$ is infeasible, which in turn accounts for the infeasibility of policy $Y$.
%\end{proof}

























%input{Rushil}


%\begin{proof}
%To prove that the policy (say $\{\textbf{p},\textbf{s},N\}$) given by Algorithm \ref{Algorithm1} is optimal, it is sufficient to show that it abides by the structure presented in Theorem \ref{th_algo1_1}.
%
%To begin with, we prove that the power allocations in Algorithm \ref{Algorithm1} are non-decreasing. We prove this by induction. The base case constitutes of showing that, the initial feasible solution has non-decreasing powers. If INIT\_POLICY returns the constant power policy from time $R$ to $S$ with power $p_c=\frac{\ETx(t_n)}{S-R}=\frac{\ETx(t_n)-\ETx(t_q^-)}{S-t_q}$, then our claim holds. 
%
%Suppose INIT\_POLICY does not return the constant power policy, but applies Algorithm 1 from \cite{Yang} with $\widetilde{B}$ bits to transmit after time $t_q$, then the transmission power after time $t_q$ is always non-decreasing. Now, we need to prove that transmission power $p_c$ between time $R$ and $t_q$ is less than or equal to the transmission power just after time $t_q$ (say $p_i$). Let transmission with $p_i$ end at epoch $t_i$. We prove it by contradiction. Assume that $p_i<p_c$. Following two cases arise.
%
%\textit{Case1:} If $t_i<S$, energy consumed by $p_c$ between time $t_q$ to $t_i$ is 
%\begin{align}
%&p_c(t_i-t_q)>p_i(t_i-t_q)=(\ETx(t_i^-)-\ETx(t_q^-))\label{eq_1_algo1_modified}
%\end{align}
%Since, constant power policy with $p_c$ uses all the available energy by $t_q$, the maximum amount of energy available for transmission between $t_q$ and $t_i$ is $\left(\ETx(t_i^-)-\ETx(t_q^-)\right)$. But by \eqref{eq_1_algo1_modified}, $p_c$ is infeasible between time $t_q$ and $t_i$. As transmitting with power $p_c$ was feasible between $t_q$ and $S$ (and therefore between $t_q$ and $t_i$) in constant power policy, we reach a contradiction.        
%
%\textit{Case2:} If $t_i>S$, then $\ETx(t_i^-)>\ETx(S)=\ETx(t_n)$. So, 
%\begin{align}
%g(p_i)(t_i-t_q)&=g\left(\frac{\ETx(t_i^-)-\ETx(t_q^-)}{t_i-t_q}\right)(t_i-t_q)
%\\
%&>g\left(\frac{\ETx(t_n)-\ETx(t_q^-)}{t_i-t_q}\right)(t_i-t_q)
%\\
%&\stackrel{(a)}{>}g\left(\frac{\ETx(t_n)-\ETx(t_q^-)}{S-t_q}\right)(S-t_q)\label{eq_2_algo1_modified}
%\\
%&=g(p_c)(S-t_q)=\widetilde{B}.
%\end{align}
%where %\eqref{eq_2_algo1_modified} 
%$(a)$ follows from \eqref{property_decreasing}. So transmission with $p_i$ from $t_q$ to $t_i$ sends more than $\widetilde{B}$ bits. This is inconsistent with the assumption that the solution we get from Algorithm 1 in \cite{Yang} exactly transmits $\widetilde{B}$ bits after $t_q$. 
%
%Now that we have proved the base case, we assume that transmission powers from Algorithm \ref{Algorithm1} are non-decreasing till its $n^{th}$ iteration. The transmission powers between $t_l$ and $t_r$ do not change from the $n^{th}$ to the $(n+1)^{th}$ iteration, as illustrated in Fig. \ref{figure_Algorithm1}. So, we only need to prove that the transmission power before time $t_l$ is less than the transmission power after $t_l$ and the same for time $t_r$. In the $(n+1)^{th}$ iteration, by the definition of the algorithm either $t_l$ updates or $t_{r}$ updates. Assume $t_l$ gets updated to $t_{l}'$, $p_l$ to $p_l'$, $p_r$ to $p_r'$ and $t_r$ remains same. The proof for $t_r$ getting updated can be done with similar arguments and hence we only show proof of this case. If we show that $p_l<p_l'$ and $p_r>p_r'$, then we are done by induction hypothesis.
%
%If $t_l$ updates and $t_r$ remains same, then we are certain that $p_{r}'>p_r$ by algorithm definition. Now, from $n^{th}$ step to $(n+1)^{th}$ step, the number of bits transmitted after $t_r$ should decrease as $p_{r}'>p_r$. So, the number of bits transmitted before $t_l$ must be increasing from $n^{th}$ to $(n+1)^{th}$ iteration. This implies that $p_l'$ must also be less than $p_l$. In the case where $p_r$ is increased till infinity, and $t_r$ and $p_r$ are updated to their previous values, the powers must remain increasing, since $p'_l <p_l$ and the remaining powers are increasing, by the induction hypothesis. Hence we have proved that the transmission powers are always non-deceasing in the policy being output by Algorithm \ref{Algorithm1}. So it follows structure \eqref{claim3}, \eqref{claim4}.
%
%%Now, we show that transmission powers follow structure \eqref{claim3}. Assume it does not. Specifically, say $p_1$ does not follow structure \eqref{claim3}. The proof for $p_2,p_3..$ can be done likewise. So, $p_1$ has to be more than the minimum possible power i.e. $p_1>\mathcal{P}(s_1,\tilde{s})$, where $\tilde{s}=\displaystyle\argmin_{t_i: s_n < t_i \le s_{N+1}} \mathcal{P}(t_i,s_n)$. Then the amount of energy used by $p_1,p_2,..$ till epoch $\tilde{s}$ can be lower bounded by $p_1(\tilde{s}-s_1)$, as $p_1>p_2..$ . But the maximum power available till time $\tilde{s}$ is $\ETx(\tilde{s})=\mathcal{P}(s_1,\tilde{s})(\tilde{s}-s_1)>p_1(\tilde{s}-s_1)$, which is more than what is spent by $p_1$. Hence we reach a contradiction and therefore $p_1=\mathcal{P}(s_1,\tilde{s})$.
%
%Next, we show that Algorithm \ref{Algorithm1} always terminates to a policy i.e it cannot continue indefinitely. The initial policy to Algorithm \ref{Algorithm1} is given by Algorithm \ref{init_policy}. If the policy output by Algorithm \ref{init_policy}, is the constant power policy returned in line \ref{init_policy_CP}, then initially $T_{stop}-T_{start}=R-S=\widetilde{\TRx}_0$, where $\widetilde{\TRx}_0$ is defined in line \ref{init_policy_CP_time}. From line \ref{init_policy_Etn} and \ref{init_policy_CP_time} of Algorithm \ref{init_policy}, 
%\begin{align}
%& \widetilde{\TRx}_0g\left(\dfrac{\ETx(t_n)}{\widetilde{\TRx}_0}\right) = B_0, \TRx_0g\left(\dfrac{\ETx(t_n)}{\TRx_0}\right) \ge B_0.
%\end{align}    
%So $\widetilde{\TRx}_0\le \TRx_0$ by \eqref{property_decreasing}. Hence $T_{stop}-T_{start}$ is initially less or equal than $\TRx_0$.
%
%If Algorithm \ref{init_policy} returns policy from line \ref{init_policy_Yang}, then by the properties satisfied by optimal policy presented in \cite{Yang}, we know that the transmission powers would be non-decreasing after time $t_q$. The policy returned by line \ref{init_policy_Yang} is same as policy in line \ref{init_policy_CP} till time $t_q$. As transmission with power $p_c$ after $t_q$ finishes transmission of $B_0$ bits till time $S$, the policy form line \ref{init_policy_Yang}, transmitting with atleast $p_c$ or more power after $t_q$, would definitely finish before time $S$. So $T_{stop}-T_{start}$ in the initial iteration of Algorithm \ref{Algorithm1} must be less than or equal to $(R-S)=\TRx_0$. So, with policy returned by INIT\_POLICY, Algorithm \ref{Algorithm1} always enters the \textbf{while} loop in line number \ref{algo_while_loop}. From the arguments presented while proving non-decreasing powers of Algorithm \ref{Algorithm1}, we can also conclude that $T_{start}$ and $T_{stop}$ always decrease across the iterations. In all the cases of Algorithm \ref{Algorithm1}, described in Fig. \ref{figure_Algorithm1} (a) (b) (d), we can show, using Lemma \ref{lemma_increase_time}, that $T_{stop}-T_{start}$ always increases across the iterations in finite steps. So after some finite number of iterations, $T_{stop}-T_{start}$ will increase beyond $\TRx_0$, or $T_{start}$ would reach 0 and Algorithm \ref{Algorithm1} would terminate from the \textbf{while} loop in line number \ref{algo_while_loop}. Hence Algorithm \ref{Algorithm1} converges.
% 
%From the arguments presented before Theorem \ref{th_algo1_1}, we know that the policy being output by Algorithm \ref{Algorithm1} follows Lemma \ref{transmission_duration} and Lemma \ref{lemma_Q}, which imply structure \eqref{claim2} and \eqref{claim5}, respectively. To conclude, all structural results \eqref{claim1}-\eqref{claim5} are satisfied by the policy output by Algorithm \ref{Algorithm1}. Therefore,  by Theorem \ref{th_algo1_1}, Algorithm \ref{Algorithm1} results in an optimal solution.
%
%%As $T_{stop}$ decreases in every iteration of the algorithm, $t_r$ must also decrease globally, though it can increase in few iterations. Hence we can be sure that $t_r$ can potentially reach $t_q$ (Initially $t_r>t_q$). If it does reach $t_q$, then the policy    
%
%
%%      
%% 
%%First we prove that the power allocations in Algorithm \ref{Algorithm1} are in accordance with \eqref{claim3}. In any particular iteration of the algorithm, we select the maximum transmission power between $t_{l}$ and all epochs before lying in range $t_{start}$ to $t_l$. Let $t_j$ be the epoch which amounts to the maximum power and $p_j$ be the maximum power, i.e. 
%%\begin{align}
%%&t_j=\argmax_{t_i:t_{start}\le t_i< t_l} \max\left(\frac{\ETx(t_l^-)-\ETx(t_i^-)}{t_l-t_i}, \frac{\ETx(t_l^-)}{t_l-t_{start}}\right)
%%\\
%%&p_j= \max_{t_i:t_{start}\le t_i< t_l} \max\left(\frac{\ETx(t_l^-)-\ETx(t_i^-)}{t_l-t_i}, \frac{\ETx(t_l^-)}{t_l-t_{start}}\right)
%%\label{eq_max_algo1_2}
%%\end{align}
%%We claim that this is indeed the maximum over all $t_i$'s in range $s_1$ to $t_l$. To prove this by contradiction, assume that $\exists t_{a}: s_1\le t_{a}<t_{start}$ and $p_{a}=\dfrac{\ETx(t_l^-)-\ETx(t_a^-)}{t_l-t_a}>p_j $. From \eqref{eq_max_algo1_2}, we can say that 
%%\begin{align}
%%&\ETx(t_l^-)\le p_j(t_l-t_{start}),\\
%%&\implies \ETx(t_l^-)<p_a(t_l-t_{start}).
%%\end{align}
%%But transmission with power $p_a$ consumes $p_a(t_l-t_{start})$ amount of energy between $t_j$ and $t_l$, which is more than the maximum available energy till $t_l$ i.e. $\ETx(t_l^-)$. Hence transmission with $p_a$ is infeasible. 
%%
%% 
%%Now we seek to show that this procedure of selecting maximum slopes going 'backwards' also gives us the minimum slopes going 'forwards', as described in \eqref{claim3}.\\
%%We shall show this by contradiction. Let $t_i$, $t_j$ and $t_k$ be three consecutive corner points where the power of transmission increases, as per our allocation. Now suppose, it is possible to transmit with a lower power between $t_i$ and some $t'_j$. 
%%Then the power of transmission between $t_j$ and $t_k$ is not the maximum power since we could transmit at a higher power from $t'_j$ and $t_k$. Which is a contradiction as this is not consistent with out allocation algorithm.\\
%%Therefore, the allocation policy before point $t_q$ is consistent with the structure.. (See figure)
%%We can prove similarly for the powers after point $t_q$.
%\end{proof}





